Discovering Unsupervised Behaviours from Full-State Trajectories

Improving open-ended learning capabilities is a promising approach to enable robots to face the unbounded complexity of the real-world. Among existing methods, the ability of Quality-Diversity algorithms to generate large collections of diverse and high-performing skills is instrumental in this context. However, most of those algorithms rely on a hand-coded behavioural descriptor to characterise the diversity, hence requiring prior knowledge about the considered tasks. In this work, we propose an additional analysis of Autonomous Robots Realising their Abilities; a Quality-Diversity algorithm that autonomously finds behavioural characterisations. We evaluate this approach on a simulated robotic environment, where the robot has to autonomously discover its abilities from its full-state trajectories. All algorithms were applied to three tasks: navigation, moving forward with a high velocity, and performing half-rolls. The experimental results show that the algorithm under study discovers autonomously collections of solutions that are diverse with respect to all tasks. More specifically, the analysed approach autonomously finds policies that make the robot move to diverse positions, but also utilise its legs in diverse ways, and even perform half-rolls.

==> algorithms/aurora.tex <==
\begin{algorithm}[t]
  \small
  \caption{\aurora{} (number of iterations $I$; encoder $\encoder$; target container size $\targetscC$, container update period $T_\cC$)}
  \label{algo:aurora}
  
  \newcommand\algorithmicitemindent{\hspace*{\algorithmicindent}\hspace*{\algorithmicindent}}
  

  \begin{algorithmic}[1]
    \State{$\metrics \gets \text{Euclidiean distance}$}
    \State{$\container \gets \emptyset$}

    \State{Initialise $\thresholdNov$}
    \For{$iter$ = 1 $\rightarrow I$}
    
    \State{$\container \gets$ \Call{QD\_Iteration}{$iter$, $\container$, $\encoder$, $\metrics$}}
    
    \If{encoder update expected at iteration $iter$} 
        \State{$\{\encoder, \container\} \gets$ \Call{Encoder\_Update}{$\encoder$, $\container$}}
    \EndIf
    \State{$\{\container, \thresholdNov\} \gets$ \Call{Manage\_Container\_Size}{$\container, \thresholdNov, \targetscC, T_\cC$}}

      \EndFor\label{auroraendfor}
      \State{\Return container $\container$}
      
\item[]
    \Procedure{QD\_Iteration}{$iter$, $\container$, $\encoder$, $\metrics$}
          \If{first iteration}
      \State{$\vect{pop_{parents}} \gets $ random()}
      \State{$\vect{pop_{offspring}} \gets $ random()}
    \Else
        \State{$\vect{pop_{parents}} \gets $ selection($\container$) }
        \State{$\vect{pop_{offspring}} \gets $ random\_variation($\vect{pop_{parents}}$) }
    \EndIf
    \ForEach{$indiv$ in $\vect{pop_{offspring}}$}
    \State{$\{\obsindiv,  \perfindiv\}  \gets$ evaluate($indiv$) }
    \State{$\bdpropindiv \gets\encoder(\obsindiv)$} 
    \State{$\container \gets$ attempt\_add\_to\_container($indiv$, $\container$, $\metrics$)} 
    \EndFor
    
    \State{\Return $\container$}
    \EndProcedure
 
\item[]
   
    \Procedure{Encoder\_Update}{$\container$, $\encoder$}
        \State{$\encoder \gets$ train($\encoder$, $\container$)}
        \State{$\container \gets$ update\_descriptors\_in\_container($\container$, $\encoder$)} 
        \State{\Return $\encoder, \container$}
    \EndProcedure
    
\item[]

    \Procedure{Manage\_Container\_Size}{$\container, \thresholdNov, \targetscC, T_\cC$}
          \State{$\thresholdNov \gets$ update\_threshold\_distance($\thresholdNov$, $\scC$, $\targetscC$) }\label{algo:aurora:update_threshold}
        \If{$iter$ multiple of $T_\cC$} 
            \State{$\container \gets$ update\_container($\container$, $\thresholdNov$)}  \label{algo:aurora:update_container}  %TODO: Provide more insights on the role played by this part. 
        \EndIf
        
        \State{\Return $\container, \thresholdNov$}
    \EndProcedure
     
  \end{algorithmic}
\end{algorithm}




==> algorithms/task_based_aurora.tex <==
\begin{algorithm}[t]
  \small
  \caption{\name{} (number of iterations $I$; encoder $\encoder$; target container size $\targetscC$, container update period $T_\cC$, downstream task execution period $T_{task}$)}
  \label{algo:task_based_aurora}
  \newcommand\algorithmicitemindent{\hspace*{\algorithmicindent}\hspace*{\algorithmicindent}}
  
  
  \begin{algorithmic}[1]
  
  \State{$\metrics \gets \text{Euclidiean distance}$}
  \State{$\container \gets \emptyset, \buffer \gets \emptyset$}
  \State{Initialise $\thresholdNov$}

  \For{$iter$ = 1 $\rightarrow I$} 
  
    \State{$\container \gets$ \Call{QD\_Iteration}{$iter$, $\container$, $\encoder$, $\metrics$}}
    
    \If{encoder update expected at iteration $iter$} 
        \State{$\{\encoder, \container\} \gets$ \Call{Encoder\_Update}{$\encoder$, $\container$}}
    \EndIf
    \State{$\{\container, \thresholdNov\} \gets$ \Call{Manage\_Container\_Size}{$\container, \thresholdNov, \targetscC, T_\cC$}}
    \item[]
    \If{$iter$ multiple of $T_{task}$}
        \State{$\vect{pop_{useful}} \gets run\_task(\container)$}
        \State{Add $\vect{pop_{useful}}$ to circular buffer $\buffer$}
        \State{$\metrics \gets update\_metrics(\buffer)$}
    \EndIf
  \EndFor
      \State{\Return container $\container$}
  \end{algorithmic}
\end{algorithm}


==> tables/downstream_tasks.tex <==
\begin{table*}[t]
    \centering
    \tiny

    \label{table:variants}

    \begin{threeparttable}
    \begin{tabular}{l l l l}
    \toprule
        Downstream Task & Task solver return & Task Score & Container Score \\
        \midrule
    	\addlinespace

    Navigation & Individuals for reaching the goal & $-1 *$(number of actions to reach goal) & $x_T,y_T$ coverage \\
    Moving forward & 10 individuals with highest $x_T$ & $\max_{ind}\left( x^{ind}_T \right)$ & $mean_{ind}\left( x^{ind}_T \right)$ \\
    Half-roll & 10 individuals with closest $\alpha_{pitch}$ to $-\frac{\pi}{2}$ & $\max_{ind} \left(-\lvert \alpha^{ind}_{pitch} - (-\frac{\pi}{2}) \rvert \right)$ & $mean_{ind} \left(-\lvert \alpha^{ind}_{pitch} - (-\frac{\pi}{2}) \rvert \right)$ \\

    \bottomrule
    	
    \end{tabular}
    
    % \begin{tablenotes}
    %      \item[1] CSC and VAT correspond respectively to the \textit{Container Size Control} and the \textit{Volume Adaptive Threshold} techniques. 
    %      \item[2] HC refers to \textit{Hand-Coded}.
    %  \end{tablenotes}
    \end{threeparttable}

\caption[Downstream tasks]{
    Description of Downstream tasks
    }
    \label{table:downstream_tasks}

\end{table*}


==> tables/hand_coded_qd_tasks.tex <==
\begin{table}[t]
    \centering
    \small

    \begin{threeparttable}
    \begin{tabular}{l l l l}
    \toprule
    & \multicolumn{2}{c}{QD Task Properties} \\ \cmidrule(lr){2-3}
        Downstream Task & Hand-coded BD & Fitness \\
        \midrule
    	\addlinespace

Navigation & $(x_T,y_T)$ & $- \left\lvert \alpha_{yaw} - \alpha_{target} \right\rvert$   \\

Moving Forward & Duty Factor & $x_T$  \\

Half-roll &  $(\alpha_{yaw}, \alpha_{roll})$  & $-\left\lvert\alpha_{pitch} - \left(-\frac{\pi}{2}\right)\right\rvert$  \\

    \bottomrule
    	
    \end{tabular}
    
    % \begin{tablenotes}
    %      \item[1] CSC and VAT correspond respectively to the \textit{Container Size Control} and the \textit{Volume Adaptive Threshold} techniques. 
    %      \item[2] HC refers to \textit{Hand-Coded}.
    %  \end{tablenotes}
    \end{threeparttable}

\caption[Hand-coded Quality-Diversity tasks]{
    Hand-coded Quality-Diversity tasks. The related downstream stask are listed in Table~\ref{table:downstream_tasks}.
    }
    \label{table:hc_qd_tasks}

\end{table}

==> tables/hyperparameters.tex <==
\begin{table}[t]
    \centering
    % \small


    \begin{threeparttable}
    \begin{tabular}{l l}
    \toprule
    Hyperparameter & Value \\
        \midrule
    	\addlinespace
    Hyperparameter & Value \\

    \bottomrule
    	
    \end{tabular}
    
    % \begin{tablenotes}
    %      \item[1] CSC and VAT correspond respectively to the \textit{Container Size Control} and the \textit{Volume Adaptive Threshold} techniques. 
    %      \item[2] HC refers to \textit{Hand-Coded}.
    %  \end{tablenotes}
    \end{threeparttable}

\caption[Hyperparameters]{
    Hyperparameters
    }
    \label{table:variants}

\end{table}


==> tables/variants.tex <==
\begin{table}[t]
    \centering
    \small

    \begin{threeparttable}
    \begin{tabular}{l l c c}
    \toprule

Variant & BD & \begin{tabular}{@{}l@{}}
                   Uses Downstream \\
                   Task Solver \\
                 \end{tabular}
                 & Has Fitness \\

        \midrule
    	\addlinespace

% \name{} & Unsupervised & \cmark & \xmark \\
AURORA & Unsupervised & \xmark & \cmark \\

% \addlinespace

% \relevantMeanStreams{} & Mean streams & \cmark & \xmark \\
\meanStreams{} & Mean streams & \xmark & \cmark \\

\addlinespace


HC & QD Task BD & \xmark & \cmark \\
% Meta Feature Maps & & & \\
% STAX & & & \\
    \bottomrule
    	
    \end{tabular}
    
    % \begin{tablenotes}
    %      \item[1] CSC and VAT correspond respectively to the \textit{Container Size Control} and the \textit{Volume Adaptive Threshold} techniques. 
    %      \item[2] HC refers to \textit{Hand-Coded}.
    %  \end{tablenotes}
    \end{threeparttable}


\caption[Summary]{Characteristics of the variants of \name{} under study, grouped based on their type of Behavioural Descriptor (BD).}
    \label{table:variants2}


\end{table}

